Alpha Decay Processes under a Diproton, Dineutron and Deuteron Pairing Scheme

In this paper we are able to justify the existence or no of photons emitted during $\alpha$ decay, based on the average half life times using the BCS superconductivity and superfluidity theories. The proposed model suggests two possible channels. A first channel where the protons and neutrons interact separately through a spin coupling, giving rise to diprotons and dineutrons which in turn interact through an isospin coupling to form an $\alpha$ particle, and a second channel where the protons and neutrons are treated as nucleons that interact through an isospin coupling, giving rise to deuterons, which in turn interact through a spin coupling to form an $\alpha$ particle. Due to the nature of the involved particles, the systems considered are homogeneous. For the second channel, the photon play a very important role for the possible escape of the $\alpha$ particle. Within these premises the half life times of a considerable number of heavy nuclei with spherical symmetry can be estimated with good experimental agreement.

==> table1.tex <==
\begin{table}
\caption{Half life times for different 
heavy spherical nuclei, calculated through 
pairing between the  diprotons and dineutrons. }\label{table1}
\begin{indented}
\item[]\begin{tabular}{@{}lll}
\br
Nucleus & $\tau_{1/2}$[theoretical]$(seg)$& $\tau_{1/2}$[experimental]$(seg)$ \\
\mr
${}^{254} Fm$ & $1.6876 \times 10^{+4}$ &$ 1.6828 \times 10^{+4} \pm 5.1937 \times 10^{+1}$\\

${}^{252} Fm$ & $1.3228 \times 10^{+5}$ & $1.3187 \times 10^{+5}\pm 2.5968 \times 10^{+2}$\\

${}^{250} Fm$ & $2.6069 \times 10^{+3}$ &$ 2.5968 \times 10^{+3} \pm  2.5969 \times 10^{+2}$\\

${}^{248} Fm$ & $5.2174 \times 10^{+1}$ &$ 5.1937 \times 10^{+1} \pm 5.7708 $\\

${}^{246} Fm$ & 1.5965 & 1.5870 $\pm$ 0.2884\\

${}^{250} Cf$ & $5.9819 \times 10^{+8}$ & $5.9510 \times 10^{+8} \pm 4.0914 \times 10^{+6}$ \\

${}^{248} Cf$ & $4.1740 \times 10^{+7}$& $4.1570 \times 10^{+7} \pm 3.4902 \times 10^{+4}$\\

${}^{246} Cf$ & $1.8620 \times 10^{+5}$ & $1.8542 \times 10^{+5} \pm 2.5969 \times 10^{+3}$\\

${}^{244} Cf$ & $1.6847 \times 10^{+3}$&$ 1.6793 \times 10^{+3} \pm  5.1937 \times 10^{+1}$\\

${}^{240} Cf$ & $9.2080 \times 10^{+1}$ & $9.1755 \times 10+1 \pm 1.2984 \times 10{+1}$\\

${}^{246} Cm$ & $2.1630 \times 10^{+11}$ &$ 2.1520 \times 10^{+11}\pm 1.0006 \times 10^{+9}$\\

${}^{244} Cm$ & $8.2708 \times 10^{+8}$ &$ 8.2349 \times 10^{+8} \pm 6.8245 \times 10^{+5}$\\

${}^{242} Cm$ & $2.0362 \times 10^{+7}$ &$ 2.0292 \times 10^{+7} \pm 4.9860 \times 10^{+5}$\\

${}^{240} Cm$ &  $3.3775 \times 10^{+6}$ & $3.3655 \times 10^{+6} \pm  2.4930 \times 10^{+4}$\\

${}^{244} Pu$ & $3.6872 \times 10^{+15}$ &$ 3.6714 \times 10^{+15} \pm 4.5496 \times 10^{+13}$\\

${}^{242} Pu$ & $1.7055 \times 10^{+13} $&$ 1.6984 \times 10^{+13} \pm 4.0947 \times 10^{+10}$\\

${}^{240} Pu$ & $3.0014 \times 10^{+11}$ & $2.9864 \times 10^{+11} \pm  5.0053 \times 10^{+8}$\\

${}^{238} Pu$ & $4.0066 \times 10^{+9} $& $3.9901 \times 10^{+9} \pm 1.3650 \times 10^{+7}$\\

${}^{236} Pu$ &  $1.3075 \times 10^{+8}$ & $1.3003 \times 10^{+8} \pm 3.6396 \times 10^{+5}$\\

${}^{238} U$  & $2.0419 \times 10^{+17}$ &$ 2.0328 \times 10^{+17} \pm 1.36401 \times 10^{+14}$\\

${}^{236} U$  & $1.0712 \times 10^{+15}$ &$ 1.0655 \times 10^{+15} \pm 1.3650 \times 10^{+12}$\\

${}^{234} U$  & $1.1232 \times 10^{+12}$ & $1.1169 \times 10^{+13} \pm 2.7298 \times 10^{+10}$\\

${}^{232} U$  & $3.1491 \times 10^{+9} $& $3.1347 \times 10^{+9} \pm 1.8200 \times 10^{+7}$\\

${}^{230} U$  & $2.6067 \times 10^{+6}$ &$ 2.5927 \times 10^{+6} \pm  2.5927 \times 10^{+4}$\\

${}^{232} Th$ & $6.4311 \times 10^{+17}$& $6.3923 \times 10^{+17} \pm 4.5497 \times 10^{+13}$\\

${}^{230} Th$ & $3.4477 \times 10^{+12} $&$ 3.4296 \times 10^{+12} \pm 7.2795 \times 10^{+8}$\\

${}^{228} Th$ & $8.7476 \times 10^{+7}$ &$ 8.704 \times 10^{+7} \pm  2.0019 \times 10^{+4}$\\

${}^{226} Th$ & $2.6594 \times 10^{+3}$ &$ 2.6487 \times 10^{+3} \pm  8.6562 $\\

${}^{224} Th$ & $1.5188$ &$ 1.5148  \pm  0.0289$\\

${}^{222} Th$ & $4.0503 \times 10^{-3}$ &$ 4.0395 \times 10^{-3} \pm  4.3281\times 10^{-4} $\\

${}^{220} Th$ & $1.4029 \times 10^{-5}$ &$ 1.3994 \times 10^{-5} \pm  8.6562\times 10^{-7} $\\

${}^{218} Th$ & $1.5789 \times 10^{-7}$ &$ 1.5725 \times 10^{-7} \pm  1.8755\times 10^{-8} $\\

${}^{216} Th$ & $0.0405 $ &$ 0.0404 \pm  2.8854\times 10^{-3} $\\

${}^{214} Th$ & $0.1455 $ &$ 0.1443 \pm 0.0369$\\

${}^{226} Ra$ & $7.3077 \times 10^{+10}$ &$ 7.2795 \times 10^{+10} \pm  3.1848 \times 10^{+8}$\\

${}^{224} Ra$ & $4.5831 \times 10^{+5}$ &$ 4.5621 \times 10^{+5} \pm  4.9859 \times 10^{+3}$\\

${}^{222} Ra$ & $5.5045 \times 10^{+1}$ &$ 5.4822 \times 10^{+1} \pm  0.7214$\\

${}^{220} Ra$ & $0.0246$ &$ 0.0245 \pm  2.884 \times 10^{-3}$\\

${}^{218} Ra$ & $3.7071 \times 10^{-5}$ &$ 3.6933 \times 10^{-5} \pm  1.5870 \times 10^{-6}$\\

${}^{216} Ra$ & $2.6323 \times 10^{-7}$ &$ 2.6257 \times 10^{-7} \pm  1.4427 \times 10^{-8}$\\

${}^{220} Rn$ & $8.0415 \times 10^{+1}$ &$ 8.0214 \times 10^{+1} \pm  0.1443$\\

${}^{218} Rn$ & $0.0507 $ &$ 0.0505 \pm  7.2135 \times 10^{-3}$\\

${}^{216} Rn$ & $6.5127 \times 10^{-5}$ &$ 6.4921 \times 10^{-5} \pm  7.2135 \times 10^{-6}$\\

${}^{214} Rn$ & $3.9050 \times 10^{-7}$ &$ 3.8953 \times 10^{-7} \pm  1.1855 \times 10^{-7}$\\

${}^{212} Rn$ & $2.0784 \times 10^{+3}$ &$ 2.0688 \times 10^{+3} \pm  1.0387 \times 10^{+2}$\\
\br
\end{tabular}
\end{indented}
\end{table}
%
\begin{table}[h]
\begin{indented}
\item[]\begin{tabular}{@{}lll}
\br
Nucleus & $\tau_{1/2}$[theoretical]$(seg)$& $\tau_{1/2}$[experimental]$(seg)$ \\
\mr
${}^{216} Po$ & $0.1677$ &$ 0.2092  \pm  2.8854 \times 10^{-3}$\\

${}^{214} Po$ & $2.3755 \times 10^{-4}$ &$ 2.3703 \times 10^{-4} \pm  2.8854 \times 10^{-6}$\\

${}^{212} Po$ & $4.3266 \times 10^{-7}$ &$ 4.3137 \times 10^{-7} \pm  2.8854 \times 10^{-9}$\\

${}^{210} Po$ & $1.7311 \times 10^{+7}$ &$ 1.7248 \times 10^{+7} \pm  2.4147 \times 10^{+2}$\\

${}^{208} Po$ & $1.2457 \times 10^{+8}$ &$ 1.3185 \times 10^{+8} \pm  9.0976 \times 10^{+4}$\\
\br
\end{tabular}
\end{indented}
\end{table}

==> table2.tex <==
\begin{table}[h]
\caption{$<n_{p}>$ y $<n_{n}>$ values adjusted [a] and calculated [c]. }\label{table2}
\begin{indented}
\item[]\begin{tabular}{@{}lll}
\br
Nucleus & $<n_{p}>$[a] &$<n_{p}>$[c]&$<n_{n}>$[a]& $<n_{n}>$[c] \\
\mr
${}^{254} Fm$ & 5,8809 & 3,2312 & 3,6270 &3,7129\\

${}^{252} Fm$ & 6,5815 & 3,0705 & 4,0138 & 3,4426\\

${}^{250} Fm$ &7,2627  & 2,6657 & 4,2611  &3,2755\\

${}^{248} Fm$ & 8,0441 & 2,3274 &5,1340 & 3,1227\\

${}^{246} Fm$ & 9,0744&  2,0368 & 6,1993 & 2,9638\\

${}^{250} Cf$ & 5,7286 & 3,8413 & 3,2972 & 3,9198\\

${}^{248} Cf$ & 6,1220 & 3,5049 & 3,3544 & 3,6822\\

${}^{246} Cf$ & 6,5154 & 3,0719 & 3,9137 & 3,4969\\

${}^{244} Cf$ & 7,0402 & 2,6799 & 4,6550 & 3,3107\\

${}^{240} Cf$ &9,1483 & 2,1417 & 6,9537 & 2,6569\\

${}^{246} Cm$ & 5,4841 & 4,2718 & 2,8137 & 4,3692\\

${}^{244} Cm$ & 5,7269 & 3,8260 & 3,1968 & 4,1814\\

${}^{242} Cm$ & 6,0709&  3,4535 & 3,6863 & 4,0314\\

${}^{240} Cm$ &  6,5565 & 3,1639 & 5,2326 & 3,2344\\

${}^{244} Pu$ & 5,0502 & 5,0732 & 2,4187 & 4,8595\\

${}^{242} Pu$ & 5,2260 & 4,6293 & 2,6999 & 4,5765\\

${}^{240} Pu$ & 5,4765 & 4,2400 & 3,0681 & 7,6351\\

${}^{238} Pu$ & 5,7886 & 3,8398 & 7,2112 & 4,0219\\

${}^{236} Pu$ & 6,1990 & 3,4533 & 4,2264 & 3,2477\\

${}^{238} U$  & 5,0830 & 5,1849 & 2,3378 & 4,9897\\

${}^{236} U$  & 5,2919&  4,7524 & 2,1300 & 4,7226\\

${}^{234} U$  & 5,5771 & 4,3302 & 2,3663 & 3,6169\\

${}^{232} U$  & 4,6303 & 4,3704 & 2,7550 & 3,4412\\

${}^{230} U$  &6,0964 & 3,2891 &3,2645  &3,2738\\

${}^{232} Th$ & 5,1165 & 5,1855 & 1,9549&  4,7046\\

${}^{230} Th$ & 5,2047 & 4,5017 & 2,3177&  4,3475\\

${}^{228} Th$ & 5,3549 & 3,8368 & 2,7918 & 4,1280\\
\br
\end{tabular}
\end{indented}
\end{table}

==> table3.tex <==
\begin{table}
  \caption{Half life times for different 
heavy spherical nuclei, calculated through 
pairing between the deuterons.}\label{table3}
\begin{indented}
\item[]\begin{tabular}{@{}lll}
\br
Nucleus & $\tau_{1/2}$[theoretical]$(seg)$& $\tau_{1/2}$[experimental]$(seg)$ \\
\mr
${}^{254} Fm$ & $1.6854 \times 10^{+4}$ &$ 1.6828 \times 10^{+4} \pm 5.1937 \times 10^{+1}$\\

${}^{252} Fm$ & $1.3207 \times 10^{+5}$ & $1.3187 \times 10^{+5} \pm 2.5968 \times 10^{+2}$\\

${}^{250} Fm$ & $2.5976 \times 10^{+3}$ & $2.5968 \times 10^{+3} \pm 2.5969 \times 10^{+2}$\\

${}^{248} Fm$ & $5.2011 \times 10^{+1} $& $5.1937 \times 10^{+1} \pm$ 5.7708\\

${}^{246} Fm$ & 1.5881 & 1.5870 $\pm$ 0.2884\\

${}^{250} Cf$ & $5.9518 \times 10^{+8}$ &$ 5.9510 \times 10^{+8} \pm 4.0914 \times 10^{+6}$ \\

${}^{248} Cf$ & $4.1634 \times 10^{+7}$ & $4.1570 \times 10^{+7} \pm 3.4902 \times 10^{+4}$\\

${}^{246} Cf$ & $7.9866 \times 10^{+4}$ & $1.8542 \times 10^{+5} \pm 2.5969 \times 10^{+3}$\\

${}^{244} Cf$ & $1.6806 \times 10^{+3}$ & $1.6793 \times 10^{+3} \pm 5.1937 \times 10^{+1}$\\

${}^{240} Cf$ & $9.1828 \times 10^{+1}$ & $9.1755 \times 10^{+1} \pm 1.2984 \times 10^{+1}$\\

${}^{246} Cm$ & $2.1530 \times 10^{+11}$ & $2.1520 \times 10^{+11} \pm 1.0006 \times 10^{+9}$\\

${}^{244} Cm$ & $8.2485 \times 10^{+8} $& $8.2349 \times 10^{+8} \pm 6.8245 \times 10^{+5}$\\

${}^{242} Cm$ & $2.0310 \times 10^{+7}$ & $2.0292 \times 10^{+7} \pm 4.9860 \times 10^{+5}$\\

${}^{240} Cm$ &  $3.3662 \times 10^{+6}$ &$ 3.3655 \times 10^{+6} \pm 2.4930 \times 10^{+4}$\\

${}^{244} Pu$ & $3.6787 \times 10^{+15}$ &$ 3.6714 \times 10^{+15} \pm 4.5496 \times 10^{+13}$\\

${}^{242} Pu$ & $1.7003 \times 10^{+13}$ & $1.6984 \times 10^{+13} \pm 4.0947 \times 10^{+10}$\\

${}^{240} Pu$ & $2.9907 \times 10^{+11}$ & $2.9864 \times 10^{+11} \pm  5.0053 \times 10^{+8}$\\

${}^{238} Pu$ & $3.9966 \times 10^{+9} $& $3.9901 \times 10^{+9} \pm 1.3650 \times 10^{+7}$\\

${}^{236} Pu$ & $ 1.3021 \times 10^{+8}$ & $1.3003 \times 10^{+8} \pm 3.6396 \times 10^{+5}$\\

${}^{238} U$  & $2.0347 \times 10^{+17}$ & $2.0328 \times 10^{+17} \pm 1.36401 \times 10^{+14}$\\

${}^{236} U$  & $1.0657 \times 10^{+15}$ & $1.0655 \times 10^{+15} \pm 1.3650 \times 10^{+12}$\\

${}^{234} U$  & $1.1185 \times 10^{+13}$ & $1.1169 \times 10^{+13} \pm 2.7298 \times 10^{+10}$\\

${}^{232} U$  & $3.1366 \times 10^{+9} $&$ 3.1347 \times 10^{+9} \pm 1.8200 \times 10^{+7}$\\

${}^{230} U$  & $2.5960 \times 10^{+6}$ & $2.5927 \times 10^{+6} \pm  2.5927 \times 10^{+4}$\\

${}^{232} Th$ & $6.4023 \times 10^{+17}$ &$ 6.3923 \times 10^{+17} \pm 4.5497 \times 10^{+13}$\\

${}^{230} Th$ & $3.4332 \times 10^{+12}$ &$ 3.4296 \times 10^{+12} \pm 7.2795 \times 10^{+8}$\\

${}^{228} Th$ & $8.7170 \times 10^{+7}$ & $8.704 \times 10^{+7} \pm 2.0019 \times 10^{+4}$\\

${}^{226} Th$ & $2.6518 \times 10^{+3}$ &$ 2.6487 \times 10^{+3} \pm  8.6562 $\\

${}^{224} Th$ & $1.5165$ &$ 1.5148  \pm  0.0289$\\

${}^{222} Th$ & $4.0437 \times 10^{-3}$ &$ 4.0395 \times 10^{-3} \pm  4.3281\times 10^{-4} $\\

${}^{220} Th$ & $1.4000 \times 10^{-5}$ &$ 1.3994 \times 10^{-5} \pm  8.6562\times 10^{-7} $\\

${}^{218} Th$ & $1.5736 \times 10^{-7}$ &$ 1.5725 \times 10^{-7} \pm  1.8755\times 10^{-8} $\\

${}^{216} Th$ & $0.0404 $ &$ 0.0404 \pm  2.8854\times 10^{-3} $\\

${}^{214} Th$ & $0.1443 $ &$ 0.1443 \pm 0.0369$\\

${}^{226} Ra$ & $7.2826 \times 10^{+10}$ &$ 7.2795 \times 10^{+10} \pm  3.1848 \times 10^{+8}$\\

${}^{224} Ra$ & $4.5665 \times 10^{+5}$ &$ 4.5621 \times 10^{+5} \pm  4.9859 \times 10^{+3}$\\

${}^{222} Ra$ & $5.4845 \times 10^{+1}$ &$ 5.4822 \times 10^{+1} \pm  0.7214$\\

${}^{220} Ra$ & $0.0245$ &$ 0.0245 \pm  2.884 \times 10^{-3}$\\

${}^{218} Ra$ & $3.6946 \times 10^{-5}$ &$ 3.6933 \times 10^{-5} \pm  1.5870 \times 10^{-6}$\\

${}^{216} Ra$ & $2.6256 \times 10^{-7}$ &$ 2.6257 \times 10^{-7} \pm  1.4427 \times 10^{-8}$\\

${}^{220} Rn$ & $8.0316 \times 10^{+1}$ &$ 8.0214 \times 10^{+1} \pm  0.1443$\\

${}^{218} Rn$ & $0.0505 $ &$ 0.0505 \pm  7.2135 \times 10^{-3}$\\

${}^{216} Rn$ & $6.4921 \times 10^{-5}$ &$ 6.4921 \times 10^{-5} \pm  7.2135 \times 10^{-6}$\\

${}^{214} Rn$ & $3.8984 \times 10^{-7}$ &$ 3.8953 \times 10^{-7} \pm  1.1855 \times 10^{-7}$\\

${}^{212} Rn$ & $2.0704 \times 10^{+3}$ &$ 2.0688 \times 10^{+3} \pm  1.0387 \times 10^{+2}$\\
\br
\end{tabular}
\end{indented}
\end{table}
%
\begin{table}[h]
\begin{indented}
\item[]\begin{tabular}{@{}lll}
\br
Nucleus & $\tau_{1/2}$[theoretical]$(seg)$& $\tau_{1/2}$[experimental]$(seg)$ \\
\mr
${}^{216} Po$ & $0.2094$ &$ 0.2092  \pm  2.8854 \times 10^{-3}$\\

${}^{214} Po$ & $2.3713 \times 10^{-4}$ &$ 2.3703 \times 10^{-4} \pm  2.8854 \times 10^{-6}$\\

${}^{212} Po$ & $4.3178 \times 10^{-7}$ &$ 4.3137 \times 10^{-7} \pm  2.8854 \times 10^{-9}$\\

${}^{210} Po$ & $1.7266 \times 10^{+7}$ &$ 1.7248 \times 10^{+7} \pm  2.4147 \times 10^{+2}$\\

${}^{208} Po$ & $1.3197 \times 10^{+8}$ &$ 1.3185 \times 10^{+8} \pm  9.0976 \times 10^{+4}$\\
\br
\end{tabular}
\end{indented}
\end{table}

==> table4.tex <==
\begin{table}[h]
  \caption{$<n_{d}>$ values adjusted [a] and calculated [c].}\label{table4}
\begin{indented}
\item[]\begin{tabular}{@{}lll}
\br
Nucleus & $<n_{d}>$[a]& $<n_{d}>$[c]  \\
\mr
${}^{254} Fm$ & 3,3449 & 3,6699 \\

${}^{252} Fm$ & 3,4475 & 3,7282\\

${}^{250} Fm$ & 3,2908 & 3,7683\\

${}^{248} Fm$ & 3,1327 & 4,1283\\

${}^{246} Fm$ & 2,9778 & 4,5815\\

${}^{250} Cf$ & 3,7178 & 3,6085\\

${}^{248} Cf$ & 3,6267 & 3,5183\\

${}^{246} Cf$ & 3,3859 & 3,7053\\

${}^{244} Cf$ & 3,2464 & 3,9828\\

${}^{240} Cf$ & 3,1580 & 4,8053\\

${}^{246} Cm$ & 3,8884 & 3,5915\\

${}^{244} Cm$ & 3,7054 & 3,6891\\

${}^{242} Cm$ & 3,5698 & 3,8589\\

${}^{240} Cm$ &  3,5246 & 4,2335\\

${}^{244} Pu$ & 4,1362 & 3,6391\\

${}^{242} Pu$ & 3,9954 & 3,6382\\

${}^{240} Pu$ & 3,8649 & 5,3516\\

${}^{238} Pu$ & 3,7424 & 5,6165\\

${}^{236} Pu$ &  3,6319 &  3,7370\\

${}^{238} U$  & 4,2362 & 3,6638\\

${}^{236} U$  & 4,1039 & 3,4263\\

${}^{234} U$  & 3,9858 & 2,9916\\

${}^{232} U$  & 3,7305 & 3,0981\\

${}^{230} U$  & 3,4910 & 3,2691\\

${}^{232} Th$ & 4,2435 & 3,3298\\

${}^{230} Th$ & 3,9312 & 3,3326\\

${}^{228} Th$ & 3,5797 & 3,4599\\
\br
\end{tabular}
\end{indented}
\end{table}
